Understanding Graph Neural Networks with Generalized Geometric Scattering Transforms

The scattering transform is a multilayered wavelet-based deep learning architecture that acts as a model of convolutional neural networks. Recently, several works have introduced generalizations of the scattering transform for non-Euclidean settings such as graphs. Our work builds upon these constructions by introducing windowed and non-windowed geometric scattering transforms for graphs based upon a very general class of asymmetric wavelets. We show that these asymmetric graph scattering transforms have many of the same theoretical guarantees as their symmetric counterparts. As a result, the proposed construction unifies and extends known theoretical results for many of the existing graph scattering architectures. In doing so, this work helps bridge the gap between geometric scattering and other graph neural networks by introducing a large family of networks with provable stability and invariance guarantees. These results lay the groundwork for future deep learning architectures for graph-structured data that have learned filters and also provably have desirable theoretical properties.

==> header.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}



\usepackage{xr}
\makeatletter
\newcommand*{\addFileDependency}[1]{
  \typeout{(#1)}
  \@addtofilelist{#1}
  \IfFileExists{#1}{}{\typeout{No file #1.}}
}
\makeatother

\newcommand*{\myexternaldocument}[1]{
    \externaldocument{#1}
    \addFileDependency{#1.tex}
    \addFileDependency{#1.aux}
}
%%% END HELPER CODE

\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Prevent itemized lists from running into the left margin inside theorems and proofs
\usepackage{enumitem}
\setlist[enumerate]{leftmargin=.5in}
\setlist[itemize]{leftmargin=.5in}

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{Asymmetric Geometric Scattering}{M. Perlmutter,  F. Gao, G. Wolf, M. Hirn}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Understanding Graph Neural Networks with Asymmetric Geometric Scattering Transforms}

% Authors: full names plus addresses.
\author{Michael Perlmutter\thanks{University of California, Los Angeles, \texttt{perlmutter@ucla.edu}} \and Feng Gao\thanks{Yale University, \texttt{f.gao@yale.edu}} \and Guy Wolf\thanks{Universit\'{e} de Montr\'{e}al and Mila -- Quebec AI Institute, \texttt{guy.wolf@umontreal.ca}} \and Matthew Hirn\thanks{Michigan State University, \texttt{mhirn@msu.edu}}}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> old/ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Prevent itemized lists from running into the left margin inside theorems and proofs
\usepackage{enumitem}
\setlist[enumerate]{leftmargin=.5in}
\setlist[itemize]{leftmargin=.5in}

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{An Example Article}{D. Doe, P. T. Frank, and J. E. Smith}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{An Example Article}

% Authors: full names plus addresses.
\author{Michael Perlmutter}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 


==> perlmutter_understanding_2023/latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> perlmutter_understanding_2023/shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{bbm}





% COMMANDS
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bd}{\mathbf{d}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bT}{\mathbf{T}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bL}{\mathbf{L}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bN}{\mathbf{N}}
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bX}{\mathbf{X}}

\newcommand{\R}{\mathbb{R}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bS}{\mathbf{S}}
%\newcommand{\bh}{\mathbf{h}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bmu}{\bm{\mu}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\pathvar}{\mathbf{p}}


% Added by Alex 
\newcommand\review[1]{\textcolor{blue}{#1}}
\newcommand\todo[1]{\textcolor{red}{[[[#1]]]}}
\usepackage{booktabs}
\usepackage{adjustbox}
\usepackage{multirow}
\newcommand{\wone}{\mathcal{W}^{(1)}_J}
\newcommand{\wtwo}{\mathcal{W}^{(2)}_J}
% End Added by Alex


%\usepackage[utf8]{inputenc}
\usepackage{mathtools}
\usepackage{amsmath}
\usepackage{amssymb}
%\usepackage{amsthm}
\usepackage{amsfonts}
%\usepackage{authblk}
\usepackage{bm} % Math packages
%\usepackage[margin=1in]{geometry}
\usepackage{color}
\usepackage{comment}
\usepackage{caption}
\usepackage{subcaption}





\usepackage{xr}
\makeatletter
\newcommand*{\addFileDependency}[1]{
  \typeout{(#1)}
  \@addtofilelist{#1}
  \IfFileExists{#1}{}{\typeout{No file #1.}}
}
\makeatother

\newcommand*{\myexternaldocument}[1]{
    \externaldocument{#1}
    \addFileDependency{#1.tex}
    \addFileDependency{#1.aux}
}
%%% END HELPER CODE

\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Prevent itemized lists from running into the left margin inside theorems and proofs
\usepackage{enumitem}
\setlist[enumerate]{leftmargin=.5in}
\setlist[itemize]{leftmargin=.5in}

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{Generalized Geometric Scattering}{M.\ Perlmutter, A.\ Tong, F.\ Gao, G.\ Wolf, M.\ Hirn}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Understanding Graph Neural Networks with Generalized Geometric Scattering Transforms}

% Authors: full names plus addresses.
\author{Michael Perlmutter\thanks{University of California, Los Angeles, \texttt{perlmutter@ucla.edu}} \and Alexander Tong\thanks{Universit\'{e} de Montr\'{e}al and Mila, \texttt{alexander.tong@mila.quebec}} \and Feng Gao\thanks{Columbia University, \texttt{fg2539@cumc.columbia.edu}} \and Guy Wolf\thanks{Universit\'{e} de Montr\'{e}al and Mila, \texttt{guy.wolf@umontreal.ca}} \and Matthew Hirn\thanks{Michigan State University, \texttt{mhirn@msu.edu}}}
%Columbia University Mailman School of Public Health}
%\email{
\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 


==> perlmutter_understanding_2023/tables/best_power_v1.tex <==
\begin{table}[ht]
\caption{Examination of the best parameters $\wone$ vs.\ $\wtwo$ and $\alpha \in \{-0.5, -0.25, 0, 0.25, 0.5\}$. Shows the number of times each setting was the best performing over 11 datasets and 10 seeds. We find that on average $\wone$ outperforms $\wtwo$ (64 to 46) and $\alpha \in \{-0.25, 0.25, 0.5\}$ outperforms $\alpha \in \{-0.5, 0.0\}$ (28 to 14).}
\centering
\begin{tabular}{lrr|r}
\toprule
$\alpha$ & $\wone$ & $\wtwo$ & Total \\
\midrule
-0.5 & 12 & 2 & 14 \\
-0.25 & 12 & 16 & 28 \\
0.0 & 8 & 5 & 13 \\
0.25 & 13 & 14 & 27 \\
0.5 & 19 & 9 & 28 \\
\midrule
Total & 64 & 46 & 110 \\
\bottomrule
\end{tabular}
\label{tab:w1_vs_2_count}
\end{table}

==> perlmutter_understanding_2023/tables/chebyshev_v1.tex <==
\begin{table}[htb]
\caption{Test accuracy $(\mu \pm \sigma)$ over 11 datasets and 10 seeds of $\wone$ scattering computation. `exact' computation of $\wone$ scattering requires an eigendecomposition of $T$ and therefore $O(n^3)$ time. Computation with the Chebyshev polynomial of order $\tau$ on a graph with $|E|$ non-zero edges takes $O(\tau (n + |E|))$ time which is efficient for sparse graphs with $|E| \approx O(n)$. We do not see a noticeable drop in performance when approximating with $\tau \in \{10, 100\}$ as compared to the exact implementation suggesting a fast implementation of approximate $\wone$ scattering using Chebyshev approximation.}
\centering
\adjustbox{max width=0.6\textwidth}{
\begin{tabular}{lrrr}
\toprule
$\tau$ & 10 & 100 & exact \\
\midrule
COLLAB & 0.692 $\pm$ 0.010 & 0.683 $\pm$ 0.012 & 0.702 $\pm$ 0.009 \\
DD & 0.685 $\pm$ 0.025 & 0.698 $\pm$ 0.024 & 0.695 $\pm$ 0.039 \\
IMDB-BINARY & 0.688 $\pm$ 0.040 & 0.666 $\pm$ 0.050 & 0.691 $\pm$ 0.031 \\
IMDB-MULTI & 0.406 $\pm$ 0.046 & 0.414 $\pm$ 0.029 & 0.398 $\pm$ 0.027 \\
MUTAG & 0.761 $\pm$ 0.074 & 0.733 $\pm$ 0.063 & 0.688 $\pm$ 0.070 \\
NCI1 & 0.653 $\pm$ 0.016 & 0.659 $\pm$ 0.029 & 0.645 $\pm$ 0.030 \\
NCI109 & 0.668 $\pm$ 0.022 & 0.628 $\pm$ 0.013 & 0.658 $\pm$ 0.023 \\
PROTEINS & 0.772 $\pm$ 0.023 & 0.799 $\pm$ 0.016 & 0.782 $\pm$ 0.022 \\
PTC MR & 0.325 $\pm$ 0.095 & 0.333 $\pm$ 0.097 & 0.387 $\pm$ 0.089 \\
REDDIT-BINARY & 0.805 $\pm$ 0.021 & 0.822 $\pm$ 0.021 & 0.814 $\pm$ 0.021 \\
REDDIT-MULTI-5K & 0.410 $\pm$ 0.013 & 0.422 $\pm$ 0.013 & 0.417 $\pm$ 0.016 \\
\midrule
Mean & 0.624 $\pm$ 0.163 & 0.624 $\pm$ 0.160 & 0.626 $\pm$ 0.151 \\
\bottomrule
\end{tabular}}
\label{tab:chebyshev}
\end{table}

==> perlmutter_understanding_2023/tables/full_raw_v4_p1.tex <==
\begin{tabular}{llllllll}
\toprule
{$\alpha$} & {model} & {COLLAB} & {DD} & {IMDB-BINARY} & {IMDB-MULTI} & {MUTAG} & {NCI1} \\
\midrule
\multirow[c]{4}{*}{-0.5} & $\wone$ ($\tau=10$) & 0.699 $\pm$ 0.005 & 0.654 $\pm$ 0.021 & \textbf{0.740 $\pm$ 0.022} & 0.384 $\pm$ 0.032 & 0.795 $\pm$ 0.064 & 0.657 $\pm$ 0.011 \\
 & $\wone$ ($\tau=100$) & 0.676 $\pm$ 0.008 & 0.721 $\pm$ 0.017 & 0.727 $\pm$ 0.021 & 0.438 $\pm$ 0.026 & 0.725 $\pm$ 0.035 & 0.681 $\pm$ 0.022 \\
 & $\wone$ (exact) & 0.706 $\pm$ 0.006 & 0.727 $\pm$ 0.013 & 0.698 $\pm$ 0.026 & 0.397 $\pm$ 0.023 & 0.600 $\pm$ 0.000 & 0.622 $\pm$ 0.006 \\
 & $\wtwo$ & 0.699 $\pm$ 0.009 & 0.660 $\pm$ 0.014 & 0.588 $\pm$ 0.012 & 0.335 $\pm$ 0.043 & 0.775 $\pm$ 0.049 & 0.651 $\pm$ 0.006 \\
\multirow[c]{4}{*}{-0.25} & $\wone$ ($\tau=10$) & 0.684 $\pm$ 0.008 & 0.683 $\pm$ 0.013 & 0.655 $\pm$ 0.036 & 0.438 $\pm$ 0.033 & 0.660 $\pm$ 0.070 & 0.642 $\pm$ 0.018 \\
 & $\wone$ ($\tau=100$) & 0.683 $\pm$ 0.007 & 0.694 $\pm$ 0.026 & 0.635 $\pm$ 0.051 & 0.389 $\pm$ 0.016 & 0.700 $\pm$ 0.062 & 0.621 $\pm$ 0.014 \\
 & $\wone$ (exact) & 0.701 $\pm$ 0.010 & 0.711 $\pm$ 0.026 & 0.692 $\pm$ 0.038 & 0.373 $\pm$ 0.014 & 0.770 $\pm$ 0.026 & 0.650 $\pm$ 0.004 \\
 & $\wtwo$ & 0.693 $\pm$ 0.007 & 0.674 $\pm$ 0.011 & 0.579 $\pm$ 0.017 & 0.401 $\pm$ 0.045 & 0.740 $\pm$ 0.039 & 0.649 $\pm$ 0.009 \\
\multirow[c]{4}{*}{0.0} & $\wone$ ($\tau=10$) & 0.686 $\pm$ 0.010 & 0.699 $\pm$ 0.017 & 0.683 $\pm$ 0.019 & \textbf{0.444 $\pm$ 0.030} & 0.750 $\pm$ 0.035 & 0.663 $\pm$ 0.022 \\
 & $\wone$ ($\tau=100$) & 0.698 $\pm$ 0.005 & 0.696 $\pm$ 0.028 & 0.695 $\pm$ 0.012 & 0.402 $\pm$ 0.014 & 0.735 $\pm$ 0.034 & 0.637 $\pm$ 0.017 \\
 & $\wone$ (exact) & 0.690 $\pm$ 0.007 & 0.714 $\pm$ 0.015 & 0.713 $\pm$ 0.021 & 0.421 $\pm$ 0.027 & 0.675 $\pm$ 0.063 & 0.638 $\pm$ 0.006 \\
 & $\wtwo$ & 0.694 $\pm$ 0.007 & 0.720 $\pm$ 0.017 & 0.584 $\pm$ 0.019 & 0.428 $\pm$ 0.016 & 0.640 $\pm$ 0.021 & 0.667 $\pm$ 0.004 \\
\multirow[c]{4}{*}{0.25} & $\wone$ ($\tau=10$) & 0.701 $\pm$ 0.010 & 0.697 $\pm$ 0.023 & 0.688 $\pm$ 0.044 & 0.423 $\pm$ 0.014 & 0.775 $\pm$ 0.026 & 0.650 $\pm$ 0.009 \\
 & $\wone$ ($\tau=100$) & 0.690 $\pm$ 0.005 & 0.686 $\pm$ 0.021 & 0.667 $\pm$ 0.012 & 0.403 $\pm$ 0.036 & 0.725 $\pm$ 0.089 & 0.682 $\pm$ 0.006 \\
 & $\wone$ (exact) & 0.705 $\pm$ 0.005 & 0.675 $\pm$ 0.041 & 0.684 $\pm$ 0.015 & 0.406 $\pm$ 0.016 & 0.690 $\pm$ 0.052 & 0.617 $\pm$ 0.011 \\
 & $\wtwo$ & 0.700 $\pm$ 0.007 & \textbf{0.732 $\pm$ 0.011} & 0.609 $\pm$ 0.032 & 0.427 $\pm$ 0.013 & \textbf{0.845 $\pm$ 0.064} & 0.658 $\pm$ 0.010 \\
\multirow[c]{4}{*}{0.5} & $\wone$ ($\tau=10$) & 0.690 $\pm$ 0.007 & 0.695 $\pm$ 0.021 & 0.680 $\pm$ 0.025 & 0.346 $\pm$ 0.027 & 0.825 $\pm$ 0.035 & 0.654 $\pm$ 0.006 \\
 & $\wone$ ($\tau=100$) & 0.670 $\pm$ 0.009 & 0.695 $\pm$ 0.015 & 0.607 $\pm$ 0.008 & 0.434 $\pm$ 0.012 & 0.780 $\pm$ 0.059 & 0.676 $\pm$ 0.008 \\
 & $\wone$ (exact) & \textbf{0.708 $\pm$ 0.006} & 0.651 $\pm$ 0.031 & 0.666 $\pm$ 0.034 & 0.395 $\pm$ 0.031 & 0.705 $\pm$ 0.055 & \textbf{0.696 $\pm$ 0.010} \\
 & $\wtwo$ & 0.705 $\pm$ 0.010 & 0.724 $\pm$ 0.021 & 0.608 $\pm$ 0.031 & 0.419 $\pm$ 0.045 & 0.590 $\pm$ 0.077 & 0.659 $\pm$ 0.011 \\
\bottomrule
\end{tabular}


==> perlmutter_understanding_2023/tables/full_raw_v4_p2.tex <==

\begin{tabular}{lllllll|l}
\toprule
& & {NCI109} & {PROTEINS} & {PTC MR} & {REDDIT-B} & {REDDIT-M} & {Mean} \\
\midrule
\multirow[c]{4}{*}{-0.5} & $\wone$ ($\tau=10$) & 0.631 $\pm$ 0.008 & 0.772 $\pm$ 0.012 & 0.422 $\pm$ 0.106 & 0.794 $\pm$ 0.009 & 0.403 $\pm$ 0.007 & 0.631 $\pm$ 0.016 \\
 & $\wone$ ($\tau=100$) & 0.627 $\pm$ 0.009 & 0.790 $\pm$ 0.014 & 0.292 $\pm$ 0.057 & 0.821 $\pm$ 0.021 & 0.412 $\pm$ 0.012 & 0.627 $\pm$ 0.008 \\
 & $\wone$ (exact) & 0.624 $\pm$ 0.010 & 0.798 $\pm$ 0.013 & 0.423 $\pm$ 0.056 & 0.789 $\pm$ 0.014 & 0.403 $\pm$ 0.007 & 0.617 $\pm$ 0.007 \\
 & $\wtwo$ & 0.663 $\pm$ 0.010 & 0.802 $\pm$ 0.016 & 0.366 $\pm$ 0.072 & 0.814 $\pm$ 0.011 & 0.416 $\pm$ 0.007 & 0.616 $\pm$ 0.012 \\
\multirow[c]{4}{*}{-0.25} & $\wone$ ($\tau=10$) & 0.661 $\pm$ 0.007 & 0.790 $\pm$ 0.027 & 0.251 $\pm$ 0.044 & 0.793 $\pm$ 0.008 & 0.406 $\pm$ 0.012 & 0.607 $\pm$ 0.008 \\
 & $\wone$ ($\tau=100$) & 0.615 $\pm$ 0.015 & 0.803 $\pm$ 0.013 & 0.286 $\pm$ 0.096 & 0.820 $\pm$ 0.023 & 0.424 $\pm$ 0.009 & 0.609 $\pm$ 0.014 \\
 & $\wone$ (exact) & 0.676 $\pm$ 0.004 & 0.791 $\pm$ 0.009 & \textbf{0.456 $\pm$ 0.020} & 0.808 $\pm$ 0.017 & 0.410 $\pm$ 0.016 & \textbf{0.640 $\pm$ 0.005} \\
 & $\wtwo$ & 0.680 $\pm$ 0.008 & 0.791 $\pm$ 0.038 & 0.402 $\pm$ 0.051 & 0.841 $\pm$ 0.007 & \textbf{0.435 $\pm$ 0.009} & 0.626 $\pm$ 0.009 \\
\multirow[c]{4}{*}{0.0} & $\wone$ ($\tau=10$) & 0.675 $\pm$ 0.009 & 0.780 $\pm$ 0.024 & 0.292 $\pm$ 0.090 & 0.791 $\pm$ 0.013 & 0.419 $\pm$ 0.006 & 0.624 $\pm$ 0.010 \\
 & $\wone$ ($\tau=100$) & 0.631 $\pm$ 0.013 & 0.797 $\pm$ 0.013 & 0.289 $\pm$ 0.069 & 0.814 $\pm$ 0.014 & 0.430 $\pm$ 0.013 & 0.620 $\pm$ 0.009 \\
 & $\wone$ (exact) & 0.641 $\pm$ 0.004 & 0.778 $\pm$ 0.024 & 0.384 $\pm$ 0.097 & 0.820 $\pm$ 0.009 & 0.419 $\pm$ 0.011 & 0.626 $\pm$ 0.012 \\
 & $\wtwo$ & 0.647 $\pm$ 0.008 & 0.783 $\pm$ 0.017 & 0.443 $\pm$ 0.054 & 0.825 $\pm$ 0.009 & 0.421 $\pm$ 0.014 & 0.623 $\pm$ 0.006 \\
\multirow[c]{4}{*}{0.25} & $\wone$ ($\tau=10$) & \textbf{0.690 $\pm$ 0.006} & 0.759 $\pm$ 0.019 & 0.294 $\pm$ 0.018 & 0.812 $\pm$ 0.011 & 0.412 $\pm$ 0.017 & 0.627 $\pm$ 0.003 \\
 & $\wone$ ($\tau=100$) & 0.627 $\pm$ 0.005 & \textbf{0.805 $\pm$ 0.007} & 0.375 $\pm$ 0.119 & \textbf{0.844 $\pm$ 0.014} & 0.418 $\pm$ 0.012 & 0.632 $\pm$ 0.013 \\
 & $\wone$ (exact) & 0.673 $\pm$ 0.004 & 0.787 $\pm$ 0.012 & 0.298 $\pm$ 0.102 & 0.842 $\pm$ 0.014 & 0.433 $\pm$ 0.018 & 0.619 $\pm$ 0.010 \\
 & $\wtwo$ & 0.654 $\pm$ 0.010 & 0.796 $\pm$ 0.019 & 0.379 $\pm$ 0.022 & 0.822 $\pm$ 0.013 & 0.398 $\pm$ 0.010 & 0.638 $\pm$ 0.008 \\
\multirow[c]{4}{*}{0.5} & $\wone$ ($\tau=10$) & 0.682 $\pm$ 0.011 & 0.758 $\pm$ 0.013 & 0.367 $\pm$ 0.083 & 0.837 $\pm$ 0.015 & 0.412 $\pm$ 0.014 & 0.631 $\pm$ 0.009 \\
 & $\wone$ ($\tau=100$) & 0.640 $\pm$ 0.007 & 0.800 $\pm$ 0.025 & 0.422 $\pm$ 0.048 & 0.812 $\pm$ 0.017 & 0.429 $\pm$ 0.012 & 0.633 $\pm$ 0.006 \\
 & $\wone$ (exact) & 0.679 $\pm$ 0.006 & 0.756 $\pm$ 0.020 & 0.370 $\pm$ 0.063 & 0.813 $\pm$ 0.010 & 0.420 $\pm$ 0.008 & 0.626 $\pm$ 0.009 \\
 & $\wtwo$ & 0.642 $\pm$ 0.005 & 0.794 $\pm$ 0.016 & 0.453 $\pm$ 0.017 & 0.795 $\pm$ 0.019 & 0.391 $\pm$ 0.006 & 0.616 $\pm$ 0.009 \\
\bottomrule
\end{tabular}

==> perlmutter_understanding_2023/tables/full_v1.tex <==
%\begin{table}[ht]
%    \caption{Full results, $(\mu \pm \sigma)$ over 10 seeds for 11 datasets with varying $\alpha$, $\{\mathcal{W}^{(1)}, \mathcal{W}^{(2)}\}$, and Chebyshev approximation of $\mathcal{W}^{(1)}$ with $10$ and $100$ degree Chebyshev polynomials.}
%    \centering
%    \adjustbox{max width=\textwidth}{
%        \input{tables/full_raw_v2}
%    }
%    \label{tab:full_results}
%\end{table}

\begin{table}[!h]
    \caption{Full results, $(\mu \pm \sigma)$ over 10 seeds for 11 datasets with varying $\alpha$, $\{\wone, \wtwo \}$, and Chebyshev approximation of $\wone$ with $10$ and $100$ degree Chebyshev polynomials.}
    \centering
    \adjustbox{max width=\textwidth}{
        \input{tables/full_raw_v4_p1}
    }
    \adjustbox{max width=\textwidth}{
        \input{tables/full_raw_v4_p2}
    }
    \label{tab:full_results}
\end{table}

==> perlmutter_understanding_2023/tables/power_v1.tex <==
\begin{table}[htb]
\caption{Test accuracy $(\mu \pm \sigma)$ over 11 datasets and 10 seeds of $\wone$ vs.\ $\wtwo$ scattering for different choices of $\alpha \in [-0.5, -0.25, 0, 0.25, 0.5]$ where $\mathbf{M} = \mathbf{D}^{\alpha}$, corresponding to $\mathbf{K} = \mathbf{D}^{-\alpha} \mathbf{T} \mathbf{D}^{\alpha}$. In most settings of $\alpha$, $\wone$ slightly outperforms $\wtwo$. This suggests $\wone$ type filters should be explored further.}
\centering
\begin{tabular}{rrr}
\toprule
$\alpha$ & {$\wone$ (exact)} & {$\wtwo$} \\
\midrule
-0.5 & \textbf{0.617 $\pm$ 0.007} & 0.616 $\pm$ 0.012 \\
-0.25 & \textbf{0.640 $\pm$ 0.005} & 0.626 $\pm$ 0.009 \\
0.0 & \textbf{0.626 $\pm$ 0.012} & 0.623 $\pm$ 0.006 \\
0.25 & 0.619 $\pm$ 0.010 & \textbf{0.638 $\pm$ 0.008} \\
0.5 & \textbf{0.626 $\pm$ 0.009} & 0.616 $\pm$ 0.009 \\
\bottomrule
\end{tabular}
\label{tab:w1_vs_2}
\end{table}



==> perlmutter_understanding_2023/tables/stats.tex <==
\begin{table}[ht]
    \caption{Dataset statistics, diameter, nodes, edges, average clustering coefficient (CC).}\label{tab:dataset_stats}
 %   \vskip 0.15in
\centering
\adjustbox{width=0.6\linewidth}{
    \begin{tabular}{lrrrrrr}
\toprule
{} &  Graphs &  Classes &  Diameter &   Nodes &    Edges &  CC \\
\midrule
COLLAB           &      5000 &          3 &      1.86 &   74.49 &  2457.22 &          0.89 \\
DD               &      1178 &          2 &     19.81 &  284.32 &   715.66 &          0.48 \\
IMDB-B     &      1000 &          2 &      1.86 &   19.77 &    96.53 &          0.95 \\
IMDB-M       &      1500 &          3 &      1.47 &   13.00 &    65.94 &          0.97 \\
MUTAG            &       188 &          2 &      8.22 &   17.93 &    19.79 &          0.00 \\
NCI1             &      4110 &          2 &     13.33 &   29.87 &    32.30 &          0.00 \\
NCI109           &      4127 &          2 &     13.14 &   29.68 &    32.13 &          0.00 \\
PROTEINS         &      1113 &          2 &     11.62 &   39.06 &    72.82 &          0.51 \\
PTC              &       344 &          2 &      7.52 &   14.29 &    14.69 &          0.01 \\
REDDIT-B    &      2000 &          2 &      8.59 &  429.63 &   497.75 &          0.05 \\
%REDDIT-12K &     11929 &         11 &      9.53 &  391.41 &   456.89 &          0.03 \\
REDDIT-5K  &      4999 &          5 &     10.57 &  508.52 &   594.87 &          0.03 \\
\bottomrule
\end{tabular}}
\vspace{-5mm}
\end{table}


